HUDD: A tool to debug DNNs for safety analysis

We present HUDD, a tool that supports safety analysis practices for systems enabled by Deep Neural Networks (DNNs) by automatically identifying the root causes for DNN errors and retraining the DNN. HUDD stands for Heatmap-based Unsupervised Debugging of DNNs, it automatically clusters error-inducing images whose results are due to common subsets of DNN neurons. The intent is for the generated clusters to group error-inducing images having common characteristics, that is, having a common root cause. HUDD identifies root causes by applying a clustering algorithm to matrices (i.e., heatmaps) capturing the relevance of every DNN neuron on the DNN outcome. Also, HUDD retrains DNNs with images that are automatically selected based on their relatedness to the identified image clusters. Our empirical evaluation with DNNs from the automotive domain have shown that HUDD automatically identifies all the distinct root causes of DNN errors, thus supporting safety analysis. Also, our retraining approach has shown to be more effective at improving DNN accuracy than existing approaches. A demo video of HUDD is available at https://youtu.be/drjVakP7jdU.

==> listings/probeExample.tex <==
%\begin{minipage}[t]{8.4cm}
\begin{lstlisting}[style=CStyle, mathescape=true, caption=Example of \APPR mutation probes (in bold)., label=lst:mutationProbes]
...
switch(message_type)
	case IfStatus:
		GetIfStatus(buffer);
		$\textbf{mutate\_FM\_IfStatus( buffer)}$;
		break;
	case IfHouseKeeping:
		GetIfHouseKeeping(buffer);
		$\textbf{mutate\_FM\_IfHK( buffer )}$;
		break;		
 ...
 \end{lstlisting}
%\end{minipage}

% 		$\textbf{\_unload\_FM(fm)}$;
% $\textbf{\_unload\_FM(fm)}$;

==> listings/selection.tex <==
% !TEX root =  ../MAIN.tex

\newcommand{\INDA}{10}
\newcommand{\INDB}{15}
\newcommand{\INDC}{5}

%\vspace{-3mm}
\begin{figure}[tb]

\begin{algorithmic}[1]

%\footnotesize
\scriptsize

\Require \emph{TS}, the test suite of the software under test
\Require \emph{Cov}, coverage information, for each test case
\Require \emph{ms}, the mutated statement
\Ensure \emph{PTS}, a list of test cases to be executed, sorted by priority
% (source inputs, follow-up inputs, output data).

\State $\mathit{TS}_m \gets$ subset of $\mathit{TS}$ that cover the mutated statement $\mathit{ms}$, based on \emph{Cov} \label{alg:prioritize:select}
\State $\mathit{PTS} \gets \mathit{new} \mathit{list}$ \textcolor{darkgray}{//this list is initially empty}
\State $\mathit{PTS} \gets$ based on \emph{Cov} select from $\mathit{TS_m}$ the test case $t$ that exercises $\mathit{ms}$ more times \label{alg:prioritize:first}
\State $\mathit{PTS} \gets \mathit{PTS} \cup t$ \textcolor{darkgray}{//include first the test case selected above}  \label{alg:prioritize:add}

\State \textbf{repeat} \label{alg:prioritize:repeat}
\State \hspace{\INDC mm} \textbf{for each} $n$ in ($\mathit{TS}_m$ - $\mathit{PTS}$) \textcolor{darkgray}{, i.e., is the set of test cases not already added to $\mathit{PTS}$} \label{alg:prioritize:notSel}
\State \hspace{\INDA mm} \textbf{for each} $t$ in $\mathit{PTS}$
\State \hspace{\INDB mm} compute the distance between $t$ and $n$
\State \hspace{\INDA mm} identify $t_n$ i.e., the test case $t$ with the minimal $d$ \label{alg:prioritize:minD}
\State \hspace{\INDC mm} among all the $t_n$ identified, select the one with the highest distance $d$ \label{alg:prioritize:selectStart}
\State \hspace{\INDC mm} \textbf{if} $d > 0$ \textcolor{darkgray}{//there is at least a test case with a different coverage}
\State \hspace{\INDA mm} \textcolor{darkgray}{//note: $n$ is the test case in the set ($\mathit{TS}_m$ - $\mathit{PTS}$) closer to $t_n$}
\State \hspace{\INDA mm} $\mathit{PTS} \gets \mathit{PTS} \cup n$ \label{alg:prioritize:selectEnd}
\State \textbf{until} $d > 0$ \label{alg:prioritize:until}

\end{algorithmic}
\vspace{-3mm}
\caption{PrioritizeAndReduce: Algorithm for prioritizing test cases}
%\vspace{-0.2cm}
\label{alg:prioritize}
\end{figure}


==> tables/actual_ms.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\caption{Actual mutation scores across subjects.}
\label{table:results:accuracy:full} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{7mm}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{9mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{19mm}@{\hspace{1pt}}|
}
\hline
\textbf{Subject}&\textbf{Mutants}&\textbf{Killed}&\textbf{Live}&\textbf{Mutation Score (\%)}\\ 
\hline
\emph{ESAIL}$_S$ & 3,536 & 2,311  & 1,225  & 65.36 \\
\LIBCSP&4,982&3,270&1,712&65.64 \\
\LIBPARAM&3,931&2,717&1,214&69.12 \\
\LIBUTIL &14,574 & 10,376 & 4,198 & 71.20 \\
\MLFS&21,375&17,484&3,981&81.80 \\
\hline
\end{tabular}

\end{table}


==> tables/case_studies.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\caption{Descriptions of subject artifacts.}
\label{table:caseStudies} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{13mm}
@{\hspace{2pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{18mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{13mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{22mm}@{\hspace{1pt}}|
p{20mm}|}
\hline
\textbf{Subject}&\textbf{LOC}&\textbf{Test suite type}&\textbf{\# Test cases}&\textbf{Statements} \textbf{coverage}\\
\hline
% \SAILCSW& 74,155 & System& 384 & 90.38\% \\
\emph{ESAIL}$_S$& 2,235 & System& 384 & 95.36\%\\
%ESAIL execution time: 8.3 hours
\LIBCSP &9,836 & Integration& 89 & 63.10\%\\
%LIBCSP execution time: 107 seconds
\LIBPARAM& 3,179 & Integration& 170 & 77.60\%\\
%LIBPARAM execution time: 50 seconds
\LIBUTIL& 10,576 & Unit& 201 & 83.20\%\\
%LIBUTIL execution time: 67 seconds
\MLFS& 5,402 & Unit& 4042 & 100.00\%\\
%MLFS execution time: 313 seconds (5.2 minutes)
%\MLFS{}{}$_V$& 5402 & 4042 & 100.00\%\\
\hline
\end{tabular}

\end{table}




==> tables/experimentsMagnitude.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\caption{Scale of experiments.}
\label{table:magnitude} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{12mm}
@{\hspace{2pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{25mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{30mm}@{\hspace{1pt}}|
p{20mm}|}
\hline
\textbf{Subject}&\textbf{Total test cases executed}&\textbf{Total execution time (minutes)}\\
\hline
\emph{ESAIL}$_S$&  302,158 & 1,624,336\\
\LIBCSP&  771,274 & 33,756\\
\LIBPARAM&  1,094,800 & 7,205\\
\LIBUTIL&  4,481,295 & 57,732\\
\MLFS&  170,303,452 & 189,633\\
\hline
\textbf{Total}&  176,952,979 & 1,912,662\\
\hline
\end{tabular}

\end{table}


==> tables/fsci.tex <==
% !TEX root =  ../MAIN.tex

\begin{table*}[htb]
\caption{Accuracy with uniform fixed-size sampling and uniform FSCI sampling.}
\label{table:results:accuracy:FSCI:sampling} 
\scriptsize
\centering
\begin{tabular}{|
>{\raggedleft\arraybackslash}p{11mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{11mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{11mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{11mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{11mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
}
\hline
\multicolumn{3}{|c|}{\textbf{\LIBCSP}}      & \multicolumn{3}{c|}{\textbf{\LIBPARAM}}      & \multicolumn{3}{c|}{\textbf{\LIBUTIL}}       & \multicolumn{3}{c|}{\textbf{\MLFS}}          & \multicolumn{3}{c|}{\textbf{\emph{ESAIL}}$_S$}       \\
\hline
\textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method} \\
\hline
100       & 9.88       & FIXED    & 100       & 10.17      & FIXED    & 100       & 7.32       & FIXED    & 100       & 7.80       & FIXED    &  100         &     8.89       &   FIXED     \\
200       & 5.86       & FIXED    & 200       & 6.12       & FIXED    & 200       & 5.73       & FIXED    & 200       & 5.20       & FIXED    &   200        &      6.14      &   FIXED     \\
300       & \textbf{4.48}       & FIXED    & 300       & 5.88       & FIXED    & 300       & 5.37       & FIXED    & 248       & \textbf{4.56}       & FSCI 0.1  &    300       &      5.53      &    FIXED    \\
364       & \textbf{4.42}       & FSCI 0.1  & 346       & \textbf{4.26}       & FSCI 0.1  & 333       & \textbf{4.73}       & FSCI 0.1  & 300       & \textbf{4.04}       & FIXED    &   366        &     \textbf{3.92}       &    FSCI 0.1    \\
400       & \textbf{5.49}       & FIXED    & 400       & \textbf{4.27}       & FIXED    & 400       & \textbf{4.45}       & FIXED    & 302       & \textbf{4.64}       & FSCI 0.09 &     400      &     \textbf{4.52}       &    FIXED    \\
447       & \textbf{3.70}       & FSCI 0.09 & 425       & \textbf{3.79}       & FSCI 0.09 & 409       & \textbf{4.08}       & FSCI 0.09 & 379       & \textbf{4.01}       & FSCI 0.08 &   449        &    \textbf{3.66}     &   FSCI 0.09    \\
500       & \textbf{3.85}       & FIXED    & 500       & \textbf{3.63}       & FIXED    & 500       & \textbf{3.80}       & FIXED    & 400       & \textbf{3.80}       & FIXED    &   500      &      \textbf{4.08}      &   FIXED     \\
564       & \textbf{3.53}       & FSCI 0.08 & 536       & \textbf{3.75}       & FSCI 0.08 & 514       & \textbf{3.94}       & FSCI 0.08 & 490       & \textbf{3.90}       & FSCI 0.07 &    567       &  \textbf{3.03}   &  FSCI 0.08      \\
600       & \textbf{3.65}       & FIXED    & 600       & \textbf{3.72}       & FIXED    & 600       & \textbf{3.29}       & FIXED    & 500       & \textbf{3.11}       & FIXED    &     600      &  \textbf{3.73}          &     FIXED   \\
700       & \textbf{3.00}       & FIXED    & 696       & \textbf{2.89}       & FSCI 0.07 & 668       & \textbf{3.99}       & FSCI 0.07 & 600       & \textbf{2.89}       & FIXED    &     700      &      \textbf{3.01}      &    FIXED    \\
734       & \textbf{3.62}       & FSCI 0.07 & 700       & \textbf{3.27}       & FIXED    & 700       & \textbf{3.30}       & FIXED    & 667       & \textbf{2.78}       & FSCI 0.06 &     738      &      \textbf{2.77}      &    FSCI 0.07    \\
800       & \textbf{2.90}       & FIXED    & 800       & \textbf{2.51}       & FIXED    & 800       & \textbf{3.26}       & FIXED    & 700       & \textbf{2.80}       & FIXED    &     800      &  \textbf{2.55}          &    FIXED    \\
900       & \textbf{3.09}       & FIXED    & 900       & \textbf{2.50}       & FIXED    & 900       & \textbf{3.04}       & FIXED    & 800       & \textbf{2.44}       & FIXED    &     900      &  \textbf{2.37}          &    FIXED    \\
994       & \textbf{3.00}       & FSCI 0.06 & 945       & \textbf{2.42}       & FSCI 0.06 & 906       & \textbf{3.28}       & FSCI 0.06 & 900       & \textbf{3.02}       & FIXED    &  998         &  \textbf{2.65}         &   FSCI 0.06     \\
1,000      & \textbf{2.41}       & FIXED    & 1,000      & \textbf{2.72}       & FIXED    & 1,000      & \textbf{2.31}       & FIXED    & 960       & \textbf{2.31}       & FSCI 0.05 & 1,000     &  \textbf{2.96}          &   FIXED     \\
1,422      & \textbf{2.44}       & FSCI 0.05 & 1,352      & \textbf{1.93}       & FSCI 0.05 & 1,298      & \textbf{2.72}       & FSCI 0.05 & 1,000      & \textbf{2.35}       & FIXED    &    1,429     &    \textbf{1.70}        &  FSCI 0.05 \\
\hline
\end{tabular}

Accurate results (i.e., $\delta_{acc} \le 5\%$) are in bold.
\end{table*}


==> tables/mass_operators.tex <==
% !TEX root =  ../MAIN.tex

\newcommand{\op}{\mathit{op}}
\newcommand{\ArithmeticSet}{ \texttt{+}, \texttt{-}, \texttt{*}, \texttt{/}, \texttt{\%} }
\newcommand{\LogicalSet}{ \texttt{&&}, \texttt{||} }
\newcommand{\RelationalSet}{ \texttt{>}, \texttt{>=}, \texttt{<}, \texttt{<=}, \texttt{==}, \texttt{!=} }
\newcommand{\BitWiseSet}{ \texttt{\&}, \texttt{|}, \land }
\newcommand{\ShiftSet}{ \texttt{>>}, \texttt{<<} }


\begin{table}[tb]
\caption{Implemented set of mutation operators.}
\label{table:operators} 
\centering
\scriptsize
\begin{tabular}{|@{}p{4mm}@{}|@{}p{1cm}@{\hspace{1pt}}|@{}p{7.1cm}@{}|}
\hline
&\textbf{Operator} & \textbf{Description$^{*}$} \\
\hline
\multirow{7}{*}{\rotatebox{90}{\emph{Sufficient Set}}}&ABS               & $\{(v, -v)\}$	\\
\cline{2-3}
&AOR               & $\{(\op_1, op_2) \,|\, \op_1, \op_2 \in \{ \ArithmeticSet \} \land \op_1 \neq \op_2 \} $       \\
&    			  & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{\texttt{+=}, \texttt{-=}, \texttt{*=}, \texttt{/=}, \texttt{\%} \texttt{=}\} \land \op_1 \neq \op_2 \} $       \\
\cline{2-3}
&ICR               & $\{i, x) \,|\, x \in \{1, -1, 0, i + 1, i - 1, -i\}\}$           \\
\cline{2-3}
&LCR               & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&\&}, || \} \land \op_1 \neq \op_2 \}$            \\
&				  & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&=}, \texttt{|=}, \texttt{\&=}\} \land \op_1 \neq \op_2 \}$            \\
&				  & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&}, \texttt{|}, \texttt{\&\&}\} \land \op_1 \neq \op_2 \}$            \\
\cline{2-3}
&ROR               & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \RelationalSet \}\}$            \\
&				  & $\{ (e, !(e)) \,|\, e \in \{\texttt{if(e)}, \texttt{while(e)}\} \}$ \\
\cline{2-3}
&SDL               & $\{(s, \texttt{remove}(s))\}$            \\
\cline{2-3}
&UOI               & $\{ (v, \texttt{--}v), (v, v\texttt{--}), (v, \texttt{++}v), (v, v\texttt{++}) \}$            \\   
\hline
\hline
\multirow{5}{*}{\rotatebox{90}{\emph{OODL}}}&AOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \ArithmeticSet \} \}$       \\ 
\cline{2-3}
&LOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \texttt{\&\&}, || \} \}$       \\ 
\cline{2-3}
&ROD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \RelationalSet \} \}$       \\ 
\cline{2-3}
&BOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \BitWiseSet \} \}$       \\ 
\cline{2-3}
&SOD               & $\{((t_1\,op\,t_2), t_1), ((t_1\,op\,t_2), t_2) \,|\, op \in \{ \ShiftSet \} \}$       \\ 
%\hline
%COR               & $\{(\op_1, \op_2) \,|\, \op_1, \op_2 \in \{ \texttt{\&\&}, \texttt{||}, \land \} \land \op_1 \neq \op_2 \}$            \\
\hline
\hline
\multirow{2}{*}{\rotatebox{90}{\emph{Other}}}&LVR			& $\{(l_1, l_2) \,|\, (l_1, l_2) \in \{(0,-1), (l_1,-l_1), (l_1, 0), $\\
&&\hspace{5mm}$(\mathit{true}, \mathit{false}), (\mathit{false}, \mathit{true})\}\}$           \\
\hline
\end{tabular}

$^{*}$Each pair in parenthesis shows how a program element is modified by the mutation operator on the left; we follow standard syntax~\cite{Kintis2018}. Program elements are literals ($l$), integer literals ($i$), boolean expressions ($e$), operators ($\op$), statements ($s$), variables ($v$), and terms ( $t_i$, which might be either variables or literals).
\end{table}


==> tables/mut_tools.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[ht]

\scriptsize
\centering
\caption{Mutation analysis tools in the literature.}
\begin{center}
\label{table:tools}
\begin{tabular}{|p{3mm}|p{25mm}|p{43mm}|}
\hline
\textbf{Ref.} & \textbf{Tool} & \textbf{Available} \\
\hline
\cite{rothermel1996experimental} & ADA mutation tool & NA\\
\cite{delamaro2001interface} &	Proteum & \url{https://github.com/magsilva/proteum} \\
\cite{chan2005fault} & SQL mutation tool (Chan) & NA \\
\cite{ma2006mujava} & MuJava & \url{https://cs.gmu.edu/~offutt/mujava/}\\
\cite{tuya2007mutating} & SQL mutation tool (Tuya) & NA\\
\cite{jia2008milu} & Milu & \url{https://github.com/yuejia/Milu/} \\
\cite{shahriar2008music} & SQL MUSIC & NA \\
\cite{shahriar2008mutation} & Function calls mutation tool & NA \\
\cite{madeyski2010judy} & Judy & NA \\
\cite{derezinska2011object} & ILMutator & NA \\
\cite{binh2012mutation}	& Simulink mutation tool & NA\\
\cite{mateo2012validating} & Bacterio & NA \\
\cite{dan2012semantic}	& Floating Point mutation tool & NA \\
\cite{just2014major}	& Major & \url{http://mutation-testing.org/} \\
\cite{grechanik2016mutation}	& jMINT & \url{https://github.com/Toparvion/jmint} \\
\cite{delgado2017assessment}	& MuCPP & \url{https://ucase.uca.es/mucpp/} \\
\cite{wang2017faster} & Accmut & \url{https://github.com/wangbo15/accmut}\\
\cite{hariri2018srciror} & SRCiror & \url{https://github.com/TestingResearchIllinois/srciror} \\
\cite{phan2018music} & MUSIC & \url{https://github.com/swtv-kaist/MUSIC} \\
\cite{denisov2018mull}	&  Mull & \url{https://github.com/mull-project/mull} \\
\cite{chekam2020muteria} & Muteria & \url{https://github.com/thierry-tct/muteria}\\
\hline
\end{tabular}
\end{center}
\end{table}%

==> tables/results_ms.tex <==
% !TEX root =  ../Main.tex

\begin{table}[htb]
\caption{\APPR Mutation Score.}
\label{table:results:mutationScore} 
\scriptsize
\centering
\begin{tabular}{|
>{\raggedleft\arraybackslash}p{14mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{26mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{15mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{15mm}@{\hspace{1pt}}|
}
\hline
\textbf{Subject}&\textbf{Predicted Equivalent}&\multicolumn{2}{c|}{\textbf{Mutation Score (\%)}}\\
&\textbf{Mutants Removed (\%)}&\textbf{Traditional}&\textbf{\APPR}\\ 
\hline
% 1225-32=1193; 2311/(2311+1193)
\SAIL{}$_{S}$&2.61&65.36&65.95\\
%$\mathit{\SAIL{}}$&&\\
% 4198-2281=1917; 10376/(10376+1917)


% 1214-770=444; 2717/(2717+444)

% 1712-371=1341; 3270/(3270+1341)
\LIBCSP{}&21.67&65.64&70.92\\
\LIBPARAM{}&63.43&69.12&85.95\\
% 3981-2699=1282; 17484/(17484+1282)
\LIBUTIL{}&54.34&71.20&84.41\\
\MLFS{}{}&69.37&81.80&93.49\\
\hline
$\textbf{Average}$&42.28&70.62&81.14\\
\hline
\end{tabular}

\end{table}

%2021-06-14
%Average MS with reduced test suite, above is with the whole TS
% 
%CSP 70.92
%LIBUTIL 84.41
%PARAM 85.95
%MLFS 93.49
%ESAIL 65.95

